Multi-orbital Kondo screening in strongly correlated polyradical nanographenes

We discuss coexistence of Kondo and spin excitation signals in tunneling spectroscopy in strongly correlated polyradical $\pi$-magnetic nanographenes on a metal surface. The Kondo signal is rationalized by a multi-orbital Kondo screening of the unpaired electrons. The fundamental processes are spin-flips of antiferromagnetic (AFM) order involving charged molecular multiplets. We introduce a~perturbative model, which provides simple rules to identify the presence of AFM channels responsible for Kondo screening. The Kondo regime is confirmed by numerical renormalization group calculations. This framework can be applied to similar strongly correlated open-shell systems.

==> aux4_SM.tex <==


